Bootstrapped Training of Score-Conditioned Generator for Offline Design of Biological Sequences

We study the problem of optimizing biological sequences, e.g., proteins, DNA, and RNA, to maximize a black-box score function that is only evaluated in an offline dataset. We propose a novel solution, bootstrapped training of score-conditioned generator (BootGen) algorithm. Our algorithm repeats a two-stage process. In the first stage, our algorithm trains the biological sequence generator with rank-based weights to enhance the accuracy of sequence generation based on high scores. The subsequent stage involves bootstrapping, which augments the training dataset with self-generated data labeled by a proxy score function. Our key idea is to align the score-based generation with a proxy score function, which distills the knowledge of the proxy score function to the generator. After training, we aggregate samples from multiple bootstrapped generators and proxies to produce a diverse design. Extensive experiments show that our method outperforms competitive baselines on biological sequential design tasks. We provide reproducible source code: \href{https://github.com/kaist-silab/bootgen}{https://github.com/kaist-silab/bootgen}.

==> algorithms/algo1_revised.tex <==
\begin{figure}[h]
\centering
\begin{minipage}[h!]{0.96\textwidth}
\centering
\begin{algorithm}[H]
\caption{Revision of \cref{alg:boot-gen}}\label{alg:revised1}
\begin{spacing}{1.05}
\begin{algorithmic}[1]
\State \textbf{Input:} Offline dataset $\mathcal{D}=\{\bm{x}_n,y_n\}_{n=1}^N$. 
%\State Update $\theta$ to maximize $\sum_{(\bm{x}, y)\in\mathcal{D}}w(y, \mathcal{D})\log p_{\theta}(\bm{x}|y)$.
\State Update $\phi$ to minimize $\sum_{(\bm{x}, y)\in\mathcal{D}}(f_{\phi}(\bm{x}) - y)^{2}$.
%\midrule
%\For{$i = 1.,,,.I$} \Comment{\textit{Pretraining Generator}}
%\State $\theta_{i+1} \leftarrow \theta_i$
%to maximize $\mathbb{E}_{(\bm{x},y) \sim p_{\text{rank}}(\mathcal{D})}\big[\text{log} p_{\theta}(\bm{x}|y)\big]$.
%\EndFor
%\State Set $\theta^{\ast} \leftarrow \theta_I$

\For{\textcolor{blue}{$j = 1, \ldots, N_{\text{gen}}$}} \Comment{Training multiple generaters}
\State Initialize $\mathcal{D}_{\text{tr}} \leftarrow \mathcal{D}=\{x_n,y_n\}_{n=1}^N$.
\For{$i = 1, \ldots, I$} 
\Comment{Rank-based weighted training}%\Comment{\textit{Bootstrapping}}
% \Statex \hspace{.2in}{\it $\triangleright$ Rank-based weighted training}
\State Update $\theta_n$ to maximize  
$\sum_{(\bm{x},y) \in \mathcal{D}_{\text{tr}}} 
w(y, \mathcal{D}_{\text{tr}}) \log p_{\textcolor{blue}{\theta_j}}(\bm{x} | y).$ 
% \Statex \hspace{.2in}{\it $\triangleright$ Bootstrapping}
\State Sample $\bm{x}^{\ast}_{\ell} \sim p_{\theta_n}(\bm{x}|y^{\dagger})$ for $\ell = 1,\ldots, L$. \Comment{Bootstrapping}
\State Set $y_{\ell}^{\ast} \leftarrow f_{\phi}(x_{\ell}^{\ast})$ for $\ell = 1,\ldots, L$. 
%    \For{$l=1,...,L_1$} 
%    \State Get $y_l^{\ast}=f_{\phi}(x_l^{\ast})$.
%    \EndFor
%\State Get sorted index $\{\pi_1,...,\pi_{L_1}\}$ \Comment{\textit{Filtering}}
% where $y_{\pi_1}\geq,...,\geq y_{\pi_{L_1}} $
\State Set $\mathcal{D}_{\text{aug}}$ as top-$K$ scoring samples in $\{\bm{x}_{\ell}^{\ast}, y_{\ell}^{\ast}\}_{\ell=1}^{L}$.
\State Set $\mathcal{D}_{\text{tr}} \leftarrow \mathcal{D}_{\text{tr}} \cup \mathcal{D}_{\text{aug}}$.
%    \For{$j = 1.,,,.J$} \Comment{\textit{Inner-loop Retraining}}
%    \State Update $\theta_{j+1} \leftarrow \theta_{j}$   
%    to maximize $\sum_{(\bm{x},y) \in \mathcal{D}_{\text{tr}}} w({\bm{x}},y) \log p_{\theta}(\bm{x} | y)$
%    \EndFor
%\State Set $\theta^{\ast} \leftarrow \theta_J$   
\EndFor
\EndFor
\State \textbf{Output:} trained score-conditioned generators~$p_{\theta_1}(\bm{x} | y),...,p_{\theta_N}(\bm{x} | y)$.
% \Statex {\it $\triangleright$ Evaluation with cross-agreement}
%\State $T \leftarrow T^{\ast}$, $D_{\text{sol}} \leftarrow \emptyset$

% \State Initialize $\mathcal{D}_{\text{samples}} \leftarrow \emptyset$.
% \For{$n = 1, \ldots, N$} 
% \State Sample $\bm{x}^{\ast}_{m} \sim p_{\theta_n}(\bm{x}|y^{\dagger})$ with temperature $T$ for $m \in [M]$. 
% \State Set $y_{m}^{\ast} \leftarrow f_{\phi}(x_{m}^{\ast})$ for $m \in [M]$.
% \State Set $\mathcal{D_{\text{sub-samples}}}$ as Top-$K'$ scoring samples in $\{\bm{x}_{m}^{\ast},
% y_{m}^{\ast}\}_{m=1}^{M}$. \Comment{Cross Aggregation}
% \State Set $\mathcal{D}_{\text{samples}} \leftarrow \mathcal{D}_{\text{samples}} \cup \mathcal{D_{\text{sub-samples}}}$ \Comment{Diversity Aggregation}
% \EndFor
% \State \textbf{Output:} $\mathcal{D}_{\text{samples}}$.
% \\\hrulefill
% \STATE \begin{center} \textcolor{gray}{\textbf{Step B: Inference with Cross-agreement}} \end{center}

% \FOR{$i=1.,,,I$}
% \STATE $x_1,...,x_N \sim p_{\theta_{t_i}}(x|r^{\ast})$
% \STATE Update $\mathcal{D}_{sol} \leftarrow \mathcal{D}_{sol} \cup \{x_{\pi_1},...x_{\pi_K}\}$, where $\{\pi_1,...,\pi_N\}$ is ascending sorted indices based on pseudo score: $r_i^{\dag} \sim p_{\phi}(r|x_i)$. 
% \ENDFOR
\end{algorithmic}
\end{spacing}
\end{algorithm}
\end{minipage}
\vspace{-10pt}
\end{figure}

==> algorithms/algo2_revised.tex <==
\begin{figure}[h]
\centering
\begin{minipage}[h!]{0.96\textwidth}
\centering
\begin{algorithm}[H]
\caption{Aggregation Strategy for Sample Generation}\label{alg:revised2}
\begin{spacing}{1.05}
\begin{algorithmic}[1]
\State \textbf{Input:} Trained score-conditioned generators~$p_{\theta_1}(\bm{x} | y),...,\textcolor{blue}{p_{\theta_{N_{\text{gen}}}}}(\bm{x} | y)$, and trained proxy function $f_{\phi}(\bm{x})$.
%

\State Initialize $\mathcal{D}_{\text{samples}} \leftarrow \emptyset$.
\For{\textcolor{blue}{$i = 1, \ldots, N_{\text{gen}}$}} 
\State Sample $\bm{x}^{\ast}_{m} \sim p_{\textcolor{blue}{\theta_i}}(\bm{x}|y^{\dagger})$ for $m \in [M]$. 
\State Set $y_{m}^{\ast} \leftarrow f_{\phi}(x_{m}^{\ast})$ for $m \in [M]$.
\State Set $\mathcal{D_{\text{sub-samples}}}$ as Top-$K$ scoring samples in $\{\bm{x}_{m}^{\ast},
y_{m}^{\ast}\}_{m=1}^{M}$. \Comment{Filtering}
\State Set $\mathcal{D}_{\text{samples}} \leftarrow \mathcal{D}_{\text{samples}} \cup \mathcal{D_{\text{sub-samples}}}$ \Comment{Diversity Aggregation}
\EndFor
\State \textbf{Output:} $\mathcal{D}_{\text{samples}}$.
% \\\hrulefill
% \STATE \begin{center} \textcolor{gray}{\textbf{Step B: Inference with Cross-agreement}} \end{center}

% \FOR{$i=1.,,,I$}
% \STATE $x_1,...,x_N \sim p_{\theta_{t_i}}(x|r^{\ast})$
% \STATE Update $\mathcal{D}_{sol} \leftarrow \mathcal{D}_{sol} \cup \{x_{\pi_1},...x_{\pi_K}\}$, where $\{\pi_1,...,\pi_N\}$ is ascending sorted indices based on pseudo score: $r_i^{\dag} \sim p_{\phi}(r|x_i)$. 
% \ENDFOR
\end{algorithmic}
\end{spacing}
\end{algorithm}
\end{minipage}
\vspace{-10pt}
\end{figure}

==> sections/back_matter/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

==> tables/diversity_comparison.tex <==
\begin{table}[t!]
\centering
\caption{Experimental results of diversity and the average value of samples.}\label{table:combination}
\vspace{0.1in}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lcccccccccccccccccc}
\toprule 
Components
& \multicolumn{2}{c}{RNA-A }         
& \multicolumn{2}{c}{RNA-B  }       
& \multicolumn{2}{c}{RNA-C }        
& \multicolumn{2}{c}{TFbind8 }            
& \multicolumn{2}{c}{UTR }          
& \multicolumn{2}{c}{GFP }            
\\
& Avg. 
& Div.
& Avg. 
& Div.
& Avg. 
& Div.
& Avg. 
& Div.
& Avg. 
& Div.
& Avg. 
& Div.
\\ \midrule
CMA-ES \cite{cma-es}
&  
&   
&           
&           
&   
& 
&  
&   
&           
&           
&   
& 
\\

CbAS \cite{cbas}
&  
&   
&           
&           
&   
& 
&  
&   
&           
&           
&   
& 
\\
Auto. CbAS \cite{auto_cbas}
&  
&   
&           
&           
&   
& 
&  
&   
&           
&           
&   
& 
\\
Grad \cite{design_bench}.                       
& 0.956   
& 4.11
& 0.956
& 4.12
& 0.956
& 4.11
& 0.956
& 4.12
& 0.956
& 4.11
& 0.956
& 4.12\\
BDI \cite{bdi}
&  
&   
&           
&           
&   
& 
&  
&   
&           
&           
&   
& 
\\GFN-AL \cite{gflownet-al}             
&  
&   
&           
&           
&   
& 
&  
&   
&           
&           
&   
& 
\\
\midrule
\ourmethod{}
& 
& 
&
& 
&  
& 
&  0.689
&  4.680
&           
&           
&   
& 
\\
\bottomrule
\end{tabular}}
\vspace{-0.05in}
\end{table}

==> tables/original_table.tex <==
\begin{table*}[h]
\centering
\caption{{Origical table of \cref{table2} which has switched report of GFP and UTR. }}\label{tab:orignal_table}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
 Method&RNA-A &RNA-B &RNA-C &TFBind8 &GFP&UTR&Avg.\\
\midrule
$\mathcal{D}$ (best) & \multicolumn{1}{c}{0.120}& \multicolumn{1}{c}{0.122}& \multicolumn{1}{c}{0.125}& \multicolumn{1}{c}{0.439}& \multicolumn{1}{c}{\textcolor{red}{0.593}}& \multicolumn{1}{c}{\textcolor{blue}{0.789}}
&0.365\\
REINFORCE \cite{design_bench}
& 0.159 $\pm$ 0.011
& 0.162 $\pm$ 0.007
& 0.177 $\pm$ 0.011
& 0.450 $\pm$ 0.017
& \textcolor{red}{0.575 $\pm$ 0.018}
& \textcolor{blue}{0.845  $\pm$ 0.003}
&0.395\\
CMA-ES \cite{cma-es} 
& 0.558 $\pm$ 0.012
& 0.531 $\pm$ 0.010
& 0.535 $\pm$ 0.012
& 0.526 $\pm$ 0.017
&  \textcolor{red}{0.497 $\pm$ 0.009} 
&  \textcolor{blue}{0.047  $\pm$ 0.000}
&0.449\\
BO-qEI \cite{bo-qel}
& 0.389 $\pm$ 0.009
& 0.397 $\pm$ 0.015
& 0.391 $\pm$ 0.012
& 0.439 $\pm$ 0.000
&  \textcolor{red}{0.571 $\pm$ 0.000}
&  \textcolor{blue}{0.246  $\pm$ 0.341}
&0.406\\
CbAS \cite{cbas} 
& 0.246 $\pm$ 0.008
& 0.267 $\pm$ 0.021
& 0.281 $\pm$ 0.015
& 0.467 $\pm$ 0.008
& \textcolor{red}{0.566 $\pm$ 0.018}
& \textcolor{blue}{0.852  $\pm$ 0.004}
&0.447\\
Auto. CbAS \cite{auto_cbas} 
& 0.241 $\pm$ 0.022
& 0.237 $\pm$ 0.009
& 0.193 $\pm$ 0.007
& 0.413 $\pm$ 0.012
& \textcolor{red}{0.563 $\pm$ 0.019}
& \textcolor{blue}{0.847  $\pm$ 0.003}
&0.420\\
MIN \cite{min} 
& 0.146 $\pm$ 0.009
& 0.143 $\pm$ 0.007
& 0.174 $\pm$ 0.007
& 0.417 $\pm$ 0.012
& \textcolor{red}{0.586 $\pm$ 0.000}
& \textcolor{blue}{0.830  $\pm$ 0.011}
&0.383\\
Grad \cite{design_bench}
& 0.473 $\pm$ 0.025
& 0.462 $\pm$ 0.016
& 0.393 $\pm$ 0.017
& 0.513 $\pm$ 0.007
& \textcolor{red}{0.611 $\pm$ 0.000}
& \textcolor{blue}{0.763  $\pm$ 0.181}
& 0.531\\
COMs \cite{com}
& 0.172 $\pm$ 0.026
& 0.184 $\pm$ 0.039
& 0.228 $\pm$ 0.061
& 0.512 $\pm$ 0.051
& \textcolor{red}{0.608 $\pm$ 0.000}
& \textcolor{blue}{0.737  $\pm$ 0.262}
&0.407\\
% ROMA \cite{roma} 
% & 
% & 
% & 
% & 0.439 $\pm$ 0.000
% & 0.592 $\pm$ 0.000
% & 0.541  $\pm$ 0.382
% &\\
GFN-AL \cite{gflownet-al} 
& 0.312 $\pm$ 0.013
& 0.300 $\pm$ 0.012
& 0.324 $\pm$ 0.009
& 0.538 $\pm$ 0.045
& \textcolor{red}{0.597 $\pm$ 0.021}
& \textcolor{blue}{0.051 $\pm$ 0.003}
&0.354\\
BDI \cite{bdi}
& 0.411 $\pm$ 0.000
& 0.308 $\pm$ 0.000
& 0.345 $\pm$ 0.000
& 0.595 $\pm$ 0.000
& \textcolor{red}{0.527  $\pm$ 0.000}
& \textcolor{blue}{0.837  $\pm$ 0.010}
& 0.504\\
\midrule
\ourmethod{}  
& \textbf{0.707} $\pm$ 0.005
& \textbf{0.717} $\pm$ 0.006
& \textbf{0.596} $\pm$ 0.006
& \textbf{0.833} $\pm$ 0.007
& \textcolor{red}{\textbf{0.701} $\pm$ 0.004}
& \textcolor{blue}{\textbf{0.853} $\pm$ 0.017} 
&\textbf{0.731}\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}


==> tables/revised_table.tex <==
\begin{table*}[h]
\centering
\caption{{Revised table for \cref{table2}}}\label{tab:revised_table}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
 Method&RNA-A &RNA-B &RNA-C &TFBind8 &GFP&UTR&Avg.\\
\midrule
$\mathcal{D}$ (best) & \multicolumn{1}{c}{0.120}& \multicolumn{1}{c}{0.122}& \multicolumn{1}{c}{0.125}& \multicolumn{1}{c}{0.439}& \multicolumn{1}{c}{\textcolor{blue}{0.789}}& \multicolumn{1}{c}{\textcolor{red}{0.593}}
&0.365\\
REINFORCE \cite{design_bench}
& 0.159 $\pm$ 0.011
& 0.162 $\pm$ 0.007
& 0.177 $\pm$ 0.011
& 0.450 $\pm$ 0.017
& \textcolor{blue}{0.845  $\pm$ 0.003}
& \textcolor{red}{0.575 $\pm$ 0.018}
&0.395\\
CMA-ES \cite{cma-es} 
& 0.558 $\pm$ 0.012
& 0.531 $\pm$ 0.010
& 0.535 $\pm$ 0.012
& 0.526 $\pm$ 0.017
&  \textcolor{blue}{0.047  $\pm$ 0.000}
&  \textcolor{red}{0.497 $\pm$ 0.009}

&0.449\\
BO-qEI \cite{bo-qel}
& 0.389 $\pm$ 0.009
& 0.397 $\pm$ 0.015
& 0.391 $\pm$ 0.012
& 0.439 $\pm$ 0.000
&  \textcolor{blue}{0.246  $\pm$ 0.341}
&  \textcolor{red}{0.571 $\pm$ 0.000}
&0.406\\
CbAS \cite{cbas} 
& 0.246 $\pm$ 0.008
& 0.267 $\pm$ 0.021
& 0.281 $\pm$ 0.015
& 0.467 $\pm$ 0.008
& \textcolor{blue}{0.852  $\pm$ 0.004}
& \textcolor{red}{0.566 $\pm$ 0.018}
&0.447\\
Auto. CbAS \cite{auto_cbas} 
& 0.241 $\pm$ 0.022
& 0.237 $\pm$ 0.009
& 0.193 $\pm$ 0.007
& 0.413 $\pm$ 0.012
& \textcolor{blue}{0.847  $\pm$ 0.003}
& \textcolor{red}{0.563 $\pm$ 0.019}
&0.420\\
MIN \cite{min} 
& 0.146 $\pm$ 0.009
& 0.143 $\pm$ 0.007
& 0.174 $\pm$ 0.007
& 0.417 $\pm$ 0.012
& \textcolor{blue}{0.830  $\pm$ 0.011}
& \textcolor{red}{0.586 $\pm$ 0.000}
&0.383\\
Grad \cite{design_bench}
& 0.473 $\pm$ 0.025
& 0.462 $\pm$ 0.016
& 0.393 $\pm$ 0.017
& 0.513 $\pm$ 0.007
& \textcolor{blue}{0.763  $\pm$ 0.181}
& \textcolor{red}{0.611 $\pm$ 0.000}
& 0.531\\
COMs \cite{com}
& 0.172 $\pm$ 0.026
& 0.184 $\pm$ 0.039
& 0.228 $\pm$ 0.061
& 0.512 $\pm$ 0.051
& \textcolor{blue}{0.737  $\pm$ 0.262}
& \textcolor{red}{0.608 $\pm$ 0.000}
&0.407\\
% ROMA \cite{roma} 
% & 
% & 
% & 
% & 0.439 $\pm$ 0.000
% & 0.592 $\pm$ 0.000
% & 0.541  $\pm$ 0.382
% &\\
GFN-AL \cite{gflownet-al} 
& 0.312 $\pm$ 0.013
& 0.300 $\pm$ 0.012
& 0.324 $\pm$ 0.009
& 0.538 $\pm$ 0.045
& \textcolor{blue}{0.051 $\pm$ 0.003}
& \textcolor{red}{0.597 $\pm$ 0.021}
&0.354\\
BDI \cite{bdi}
& 0.411 $\pm$ 0.000
& 0.308 $\pm$ 0.000
& 0.345 $\pm$ 0.000
& 0.595 $\pm$ 0.000
& \textcolor{blue}{0.837  $\pm$ 0.010} 
& \textcolor{red}{0.527  $\pm$ 0.000}
& 0.504\\
\midrule
\ourmethod{}  
& \textbf{0.707} $\pm$ 0.005
& \textbf{0.717} $\pm$ 0.006
& \textbf{0.596} $\pm$ 0.006
& \textbf{0.833} $\pm$ 0.007
& \textcolor{blue}{\textbf{0.853} $\pm$ 0.017} 
& \textcolor{red}{\textbf{0.701} $\pm$ 0.004}
&\textbf{0.731}\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}


==> tables/table1.tex <==
\begin{table*}[t]
\fontsize{9.0}{9.0}\selectfont
\centering
\caption{{Experimental results on median score.}}\label{table1}
\begin{tabular}{lcccccc}
\specialrule{1pt}{0pt}{4pt}
\begin{tabular}{c}\multirow{2}{*}{Method}\end{tabular}&\multicolumn{1}{c}{Protein Task}&\multicolumn{3}{c}{DNA Task}&\multicolumn{2}{c}{RNA Task}
\\\cmidrule[0.5pt](lr{0.2em}){2-2}\cmidrule[0.5pt](lr{0.2em}){3-5}\cmidrule[0.5pt](lr{0.2em}){6-7}
 &GFP & UTR & SIX6-REF-R1 & SIX6-REF-R2 & L14-RNA1 & L14-RNA2 \\
\specialrule{0.5pt}{2pt}{4pt}
$\mathcal{D}$ (best) & 0.789& 0.593 &0.439 & & & \\
BO-QEI \citep{bo-qel}& 0.246  $\pm$ 0.341 & 0.571 $\pm$ 0.000& 0.439 $\pm$ 0.000 &-- &-- &-- \\
CMA-ES \citep{cma-es}& 0.047  $\pm$ 0.000 & 0.612 $\pm$ 0.000 & 0.537 $\pm$ 0.014 &-- &-- &-- \\
REINFORCE \citep{reinforce}& 0.844  $\pm$ 0.003& 0.568 $\pm$ 0.000& 0.462 $\pm$ 0.021 &-- &-- &-- \\
CbAS \citep{cbas}& 0.848  $\pm$ 0.004& 0.572 $\pm$ 0.000& 0.428 $\pm$ 0.010&-- &-- &-- \\
Auto.CbAS \citep{auto_cbas}& 0.848  $\pm$ 0.007& 0.576 $\pm$ 0.000& 0.419 $\pm$ 0.000&-- &-- &-- \\
MIN \citep{min}& 0.427  $\pm$ 0.012& 0.586 $\pm$ 0.000& 0.421 $\pm$ 0.015&-- &-- &-- \\
Grad \citep{design_bench}& 0.836  $\pm$ 0.000& 0.611 $\pm$ 0.000& 0.439 $\pm$ 0.000&-- &-- &-- \\
COMs \citep{com}&0.737  $\pm$ 0.262& 0.608 $\pm$ 0.000& 0.512 $\pm$ 0.051&-- &-- &-- \\
ROMA \citep{roma}&0.541  $\pm$ 0.382& 0.592 $\pm$ 0.000& 0.439 $\pm$ 0.000&-- &-- &-- \\
NEMO \citep{nemo}&0.146  $\pm$ 0.260& 0.590 $\pm$ 0.000& 0.439 $\pm$ 0.000&-- &-- &-- \\
\specialrule{0.5pt}{2pt}{4pt}
GFlowNet-AL \citep{gflownet-al} & & & 0.841 $\pm$ 0.000 &  & & \\
BDI \citep{bdi}&0.860  $\pm$ 0.000&0.664  $\pm$ 0.708& 0.595 $\pm$ 0.000 & 0.519 & 0.586 & 0.560\\
\specialrule{0.5pt}{2pt}{4pt}
CC-LSTM (ours) & \textbf{0.864} $\pm$ 0.000 & \textbf{0.812} $\pm$ 0.000& \textbf{0.901} $\pm$ 0.000 & 0.780 & 0.778 & 0.848\\
\specialrule{1pt}{4pt}{-7pt}
\end{tabular}
\end{table*}


==> tables/table1_1.tex <==
\begin{table*}[h]
\centering
\caption{{Experimental results on percentile 50 score of GFP, UTR, and TFBind8-A. The best-scored value is marked in bold. }}\label{table1}
\begin{tabular}{lccc}
\toprule

 Method&GFP & UTR & TFBind8-A \\
\specialrule{0.5pt}{2pt}{4pt}
$\mathcal{D}$ (best) & 0.789& 0.593 &0.439 \\
BO-QEI \citep{bo-qel}& 0.246  $\pm$ 0.341 & 0.571 $\pm$ 0.000& 0.439 $\pm$ 0.000  \\
CMA-ES \citep{cma-es}& 0.047  $\pm$ 0.000 & 0.612 $\pm$ 0.000 & 0.537 $\pm$ 0.014 \\
REINFORCE \citep{reinforce}& 0.844  $\pm$ 0.003& 0.568 $\pm$ 0.000& 0.462 $\pm$ 0.021 \\
CbAS \citep{cbas}& 0.848  $\pm$ 0.004& 0.572 $\pm$ 0.000& 0.428 $\pm$ 0.01\\
Auto.CbAS \citep{auto_cbas}& 0.848  $\pm$ 0.007& 0.576 $\pm$ 0.000& 0.419 $\pm$ 0.000 \\
MIN \citep{min}& 0.427  $\pm$ 0.012& 0.586 $\pm$ 0.000& 0.421 $\pm$ 0.015 \\
Grad \citep{design_bench}& 0.836  $\pm$ 0.000& 0.611 $\pm$ 0.000& 0.439 $\pm$ 0.000 \\
COMs \citep{com}&0.737  $\pm$ 0.262& 0.608 $\pm$ 0.000& 0.512 $\pm$ 0.051 \\
ROMA \citep{roma}&0.541  $\pm$ 0.382& 0.592 $\pm$ 0.000& 0.439 $\pm$ 0.000 \\
NEMO \citep{nemo}&0.146  $\pm$ 0.260& 0.590 $\pm$ 0.000& 0.439 $\pm$ 0.000 \\
\midrule
GFlowNet-AL \citep{gflownet-al} & & & 0.841 $\pm$ 0.000 \\
BDI \citep{bdi}&0.860  $\pm$ 0.000&0.664  $\pm$ 0.708& 0.595 $\pm$ 0.000 \\
\midrule
Boot-Gen (ours) & \textbf{0.864} $\pm$ 0.000 & \textbf{0.834} $\pm$ 0.000& \textbf{0.884} $\pm$ 0.005 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/table1_2.tex <==
\begin{table*}[t!]
\centering
\caption{{Experimental results on 50th percentile scores (50th Per.) and 100th percentile scores (100th Per.) of GFP, UTR, and TFBind8. The mean and standard deviation are reported for 8 independent solution generations. $\mathcal{D} (\text{best})$ indicate the maximum score of the offline dataset. The best-scored value is marked in bold. $^{\dagger}$We re-use the numbers reported by \citet{bdi}.    }}\label{table1}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{GFP}& \multicolumn{2}{c}{UTR}& \multicolumn{2}{c}{TFBind8}\\
\cmidrule(lr{0.2em}){2-3}
\cmidrule(lr{0.2em}){4-5}
\cmidrule(lr{0.2em}){6-7}
 Method&50th Per. &100th Per. &50th Per. &100th Per.&50th Per. &100th Per.\\
\midrule
$\mathcal{D}$ (best) & \multicolumn{2}{c}{0.789}& \multicolumn{2}{c}{0.593}& \multicolumn{2}{c}{0.439}\\
CMA-ES \cite{cma-es} & 0.047  $\pm$ 0.000 
&0.054 $\pm$ 0.002 
& 0.612 $\pm$ 0.000 
& 0.707 $\pm$ 0.014
& 0.537 $\pm$ 0.014 
&0.953 $\pm$ 0.022\\
BO-qEI \cite{bo-qel}& 0.246  $\pm$ 0.341 
& 0.254 $\pm$ 0.352
& 0.571 $\pm$ 0.000
& 0.684 $\pm$ 0.000
& 0.439 $\pm$ 0.000 
& 0.798 $\pm$ 0.083\\
% REINFORCE$^{\dagger}$ & 0.844  $\pm$ 0.003
% & \textbf{0.865} $\pm$ 0.000
% & 0.568 $\pm$ 0.000
% & 0.688 $\pm$ 0.010
% & 0.462 $\pm$ 0.021 
% &0.948 $\pm$ 0.028\\
CbAS \cite{cbas} & 0.848  $\pm$ 0.004
& \textbf{0.865} $\pm$ 0.000
& 0.572 $\pm$ 0.000
& 0.694 $\pm$ 0.010
& 0.428 $\pm$ 0.010
&0.927 $\pm$ 0.051\\
Auto. CbAS \cite{auto_cbas} & 0.848  $\pm$ 0.007
& \textbf{0.865} $\pm$ 0.000
& 0.576 $\pm$ 0.000
& 0.691 $\pm$ 0.012
& 0.419 $\pm$ 0.000
&0.910 $\pm$ 0.044\\
MIN \cite{min} & 0.427  $\pm$ 0.012
& \textbf{0.865} $\pm$ 0.001
& 0.586 $\pm$ 0.000
& 0.694 $\pm$ 0.017
& 0.421 $\pm$ 0.015
&0.882 $\pm$ 0.020\\
% Grad$^{\dagger}$& 0.836  $\pm$ 0.000
% & 0.864 $\pm$ 0.001 
% & 0.611 $\pm$ 0.000
% & 0.666 $\pm$ 0.013
% & 0.439 $\pm$ 0.000
% &0.491 $\pm$ 0.042\\
COMs \cite{com}&0.737  $\pm$ 0.262
& 0.861 $\pm$ 0.009
& 0.608 $\pm$ 0.000
& 0.699 $\pm$ 0.011
& 0.512 $\pm$ 0.051
&0.920 $\pm$ 0.043\\
ROMA \cite{roma} &0.541  $\pm$ 0.382
& 0.558 $\pm$ 0.395  
& 0.592 $\pm$ 0.000
& 0.690 $\pm$ 0.012
& 0.439 $\pm$ 0.000
&0.928 $\pm$ 0.038\\
% NEMO$^{\dagger}$ &0.146  $\pm$ 0.260
% &0.150 $\pm$ 0.270 
% & 0.590 $\pm$ 0.000
% & 0.694 $\pm$ 0.015
% & 0.439 $\pm$ 0.000
% &0.905 $\pm$ 0.048 \\
GFN-AL \cite{gflownet-al} & 0.051 $\pm$ 0.003
& 0.059 $\pm$ 0.006
& 0.597 $\pm$ 0.021
& 0.695 $\pm$ 0.021
& 0.538 $\pm$ 0.045
&0.956 $\pm$ 0.018\\
BDI \cite{bdi}&0.860  $\pm$ 0.010
& 0.864 $\pm$ 0.000 
&0.664  $\pm$ 0.000
& 0.760 $\pm$ 0.000
& 0.595 $\pm$ 0.000
&0.973 $\pm$ 0.000 \\
\midrule
\ourmethod{}  & \textbf{0.862 $\pm$ 0.000} 
& \textbf{0.865} $\pm$ 0.000
& \textbf{0.858} $\pm$ 0.001
& \textbf{0.863} $\pm$ 0.000
& \textbf{0.866} $\pm$ 0.003 
& \textbf{0.976} $\pm$ 0.006 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/table2.tex <==
\begin{table*}[t]
\fontsize{9.0}{9.0}\selectfont
\centering
\caption{{Experimental results on top1 score among 128 samples.}}\label{table2}
\begin{tabular}{lcccccc}
\specialrule{1pt}{0pt}{4pt}
\begin{tabular}{c}\multirow{2}{*}{Method}\end{tabular}&\multicolumn{1}{c}{Protein Task}&\multicolumn{3}{c}{DNA Task}&\multicolumn{2}{c}{RNA Task}
\\\cmidrule[0.5pt](lr{0.2em}){2-2}\cmidrule[0.5pt](lr{0.2em}){3-5}\cmidrule[0.5pt](lr{0.2em}){6-7}
 &GFP & UTR & SIX6-REF-R1 & SIX6-REF-R2 & L14-RNA1 & L14-RNA2 \\
\specialrule{0.5pt}{2pt}{4pt}
$\mathcal{D}$(best) & 0.789 & 0.593& 0.439 & & & \\
BO-QEI \citep{bo-qel}& 0.254 $\pm$ 0.352& 0.684 $\pm$ 0.000& 0.798 $\pm$ 0.083 &-- &-- &-- \\
CMA-ES \citep{cma-es}&0.054 $\pm$ 0.002 & 0.707 $\pm$ 0.014&0.953 $\pm$ 0.022&-- &-- &-- \\
REINFORCE \citep{reinforce} & \textbf{0.865 $\pm$ 0.000} & 0.688 $\pm$ 0.010&0.948 $\pm$ 0.028&-- &-- &-- \\
CbAS \citep{cbas} & \textbf{0.865 $\pm$ 0.000} & 0.694 $\pm$ 0.010&0.927 $\pm$ 0.051 &-- &-- &-- \\
Auto.CbAS \citep{auto_cbas} & \textbf{0.865 $\pm$ 0.000} & 0.691 $\pm$ 0.012&0.910 $\pm$ 0.044 &-- &-- &-- \\
MIN \citep{min} & \textbf{0.865 $\pm$ 0.001} & 0.694 $\pm$ 0.017&0.882 $\pm$ 0.020 &-- &-- &-- \\
Grad \cite{design_bench} & 0.864 $\pm$ 0.001 & 0.666 $\pm$ 0.013&0.491 $\pm$ 0.042 &-- &-- &-- \\
COMs \cite{com} & 0.861 $\pm$ 0.009& 0.699 $\pm$ 0.011&0.920 $\pm$ 0.043&-- &-- &-- \\
ROMA \cite{roma} & 0.558 $\pm$ 0.395  & 0.690 $\pm$ 0.012&0.928 $\pm$ 0.038 &-- &-- &-- \\
NEMO \cite{nemo} &0.150 $\pm$ 0.270 & 0.694 $\pm$ 0.015&0.905 $\pm$ 0.048&-- &-- &-- \\
\specialrule{0.5pt}{2pt}{4pt}
GFlowNet-AL \cite{gflownet-al} & &&0.948 $\pm$ 0.000 & & & \\
BDI \cite{bdi}& 0.864$\pm$ 0.000 & 0.760 $\pm$ 0.000&0.973 $\pm$ 0.000 & 0.956 & 0.752 & 0.906 \\
\specialrule{0.5pt}{2pt}{4pt}
CC-LSTM (ours) & \textbf{0.865 $\pm$ 0.000} & \textbf{0.854 $\pm$ 0.000}& \textbf{0.974 $\pm$ 0.002} & 0.985 & 0.928 & 1.000\\
\specialrule{1pt}{4pt}{-7pt}
\end{tabular}
\end{table*}

==> tables/table2_1.tex <==
\begin{table*}[t]
\centering
\caption{{Experimental results on percentile 100 scores of GFP, UTR, and TFBind8-A. The best-scored value is marked in bold.}}\label{table2}
\begin{tabular}{lccc}
\toprule
Method&GFP & UTR & TFBind8-A \\
\midrule
$\mathcal{D}$ (best) & 0.789 & 0.593& 0.439 \\
BO-QEI \citep{bo-qel}& 0.254 $\pm$ 0.352
& 0.684 $\pm$ 0.000
& 0.798 $\pm$ 0.083 \\
CMA-ES \citep{cma-es}&0.054 $\pm$ 0.002 
& 0.707 $\pm$ 0.014
&0.953 $\pm$ 0.022\\
REINFORCE \citep{reinforce} & \textbf{0.865 $\pm$ 0.000} 
& 0.688 $\pm$ 0.010
&0.948 $\pm$ 0.028\\
CbAS \citep{cbas} & \textbf{0.865 $\pm$ 0.000} 
& 0.694 $\pm$ 0.010
&0.927 $\pm$ 0.051\\
Auto.CbAS \citep{auto_cbas} & \textbf{0.865 $\pm$ 0.000} 
& 0.691 $\pm$ 0.012
&0.910 $\pm$ 0.044\\
MIN \citep{min} & \textbf{0.865 $\pm$ 0.001} 
& 0.694 $\pm$ 0.017
&0.882 $\pm$ 0.020\\
Grad \cite{design_bench} & 0.864 $\pm$ 0.001 
& 0.666 $\pm$ 0.013
&0.491 $\pm$ 0.042  \\
COMs \cite{com} & 0.861 $\pm$ 0.009
& 0.699 $\pm$ 0.011
&0.920 $\pm$ 0.043 \\
ROMA \cite{roma} & 0.558 $\pm$ 0.395  
& 0.690 $\pm$ 0.012
&0.928 $\pm$ 0.038  \\
NEMO \cite{nemo} &0.150 $\pm$ 0.270 
& 0.694 $\pm$ 0.015
&0.905 $\pm$ 0.048 \\
\midrule
GFlowNet-AL \cite{gflownet-al} &
&
&0.948 $\pm$ 0.000 \\
BDI \cite{bdi}& 0.864$\pm$ 0.000 
& 0.760 $\pm$ 0.000
&0.973 $\pm$ 0.000  \\
\midrule
BootGen (ours) & \textbf{0.865 $\pm$ 0.000}
& \textbf{0.846 $\pm$ 0.002}
& \textbf{0.974 $\pm$ 0.002} \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/table3.tex <==



==> tables/table3_1.tex <==
\begin{table*}[t!]
\centering
\caption{Experimental results on 50th percentile scores (50th Per.) and 100th percentile scores (100th Per.) of RNA-Binding-A, RNA-Binding-B and RNA-Binding-C. The best score is marked in bold. The mean and the standard deviation are reported using eight independent runs.}\label{table2}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{RNA-Binding-A}& \multicolumn{2}{c}{RNA-Binding-B}& \multicolumn{2}{c}{RNA-Binding -C}\\
\cmidrule(lr{0.2em}){2-3}
\cmidrule(lr{0.2em}){4-5}
\cmidrule(lr{0.2em}){6-7}
 Method&50th Per.&100th Per.&50th Per.&100th Per.&50th Per.&100th Per.\\
\midrule
$\mathcal{D}$ (best) & \multicolumn{2}{c}{0.500}& \multicolumn{2}{c}{0.499}& \multicolumn{2}{c}{0.497}\\
% BO-qEI&  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% &  $\pm$  
% &  $\pm$ \\
% CMA-ES &   $\pm$ 
% & $\pm$ 
% &  $\pm$  
% &  $\pm$ 
% &  $\pm$  
% & $\pm$ \\
% REINFORCE &   $\pm$ 
% &  $\pm$ 
% & $\pm$ 
% &  $\pm$ 
% &  $\pm$  
% & $\pm$ \\
% CbAS &  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% &$\pm$ \\
% Auto. CbAS &  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% &$\pm$ \\
% MIN &  $\pm$ 
% &  $\pm$ 
% & $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% & $\pm$ \\
% Grad&  $\pm$ 
% &  $\pm$  
% &  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% & $\pm$ \\
% COMs&  $\pm$ 
% &  $\pm$ 
% &  $\pm$ 
% & $\pm$ 
% &  $\pm$ 
% &$\pm$ \\
GFN-AL & 0.500 $\pm$ 0.000
& 0.679 $\pm$ 0.044
& 0.499 $\pm$ 0.000
& 0.654 $\pm$ 0.022
& 0.497 $\pm$ 0.000
& 0.710 $\pm$ 0.070
\\
BDI
& 0.586 $\pm$ 0.000
& 0.752 $\pm$ 0.000
&0.560  $\pm$ 0.000
&0.906 $\pm$ 0.000
&0.467  $\pm$ 0.000
& 0.885$\pm$ 0.000 
\\
\midrule
\ourmethod{}  
& \textbf{ 0.716}$\pm$ 0.009
& \textbf{ 0.945} $\pm$ 0.030
& \textbf{0.712} $\pm$ 0.008
& \textbf{0.948} $\pm$ 0.049
& \textbf{0.643} $\pm$ 0.014
& \textbf{0.898} $\pm$ 0.008 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/table4_1.tex <==
\begin{table*}[h]
\fontsize{9.0}{9.0}\selectfont
\centering
\caption{{Experimental results on pecentile 50 score among 128 samples.}}\label{table3}
\begin{tabular}{lccc}
\specialrule{1pt}{0pt}{4pt}
Method&TFBind8-B & RNA-A & RNA-B \\
\specialrule{0.5pt}{2pt}{4pt}
$\mathcal{D}$(best) &&& \\
BDI \cite{bdi}& & &  \\
\specialrule{0.5pt}{2pt}{4pt}
Boot-Gen (ours) &&& \\
\specialrule{1pt}{4pt}{-7pt}
\end{tabular}
\end{table*}
